Similarity Analysis of Self-Supervised Speech Representations

Self-supervised speech representation learning has recently been a prosperous research topic. Many algorithms have been proposed for learning useful representations from large-scale unlabeled data, and their applications to a wide range of speech tasks have also been investigated. However, there has been little research focusing on understanding the properties of existing approaches. In this work, we aim to provide a comparative study of some of the most representative self-supervised algorithms. Specifically, we quantify the similarities between different self-supervised representations using existing similarity measures. We also design probing tasks to study the correlation between the models' pre-training loss and the amount of specific speech information contained in their learned representations. In addition to showing how various self-supervised models behave differently given the same input, our study also finds that the training objective has a higher impact on representation similarity than architectural choices such as building blocks (RNN/Transformer/CNN) and directionality (uni/bidirectional). Our results also suggest that there exists a strong correlation between pre-training loss and downstream performance for some self-supervised algorithms.

==> Self-Supervised Speech Analysis (ICASSP 2021)/refs-fullname.tex <==
@inproceedings{blandon2020analysis,
  title     = {Analysis of predictive coding models for phonemic representation learning in small datasets},
  author    = {Bland{\'o}n, Mar{\'\i}a Andrea Cruz and R{\"a}s{\"a}nen, Okko},
  booktitle = {ICML SAS Workshop},
  year      = {2020}
}

@inproceedings{riviere2020unsupervised,
  title     = {Unsupervised pretraining transfers well across languages},
  author    = {Rivi{\`e}re, Morgane and Joulin, Armand and Mazar{\'e}, Pierre-Emmanuel and Dupoux, Emmanuel},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{wang2020unsupervised,
  title     = {Unsupervised pre-training of bidirectional speech encoders via masked reconstruction},
  author    = {Wang, Weiran and Tang, Qingming and Livescu, Karen},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{liu2020mockingjay,
  title     = {Mockingjay: Unsupervised speech representation learning with deep bidirectional {Transformer} encoders},
  author    = {Liu, Andy and Yang, Shu-Wen and Chi, Po-Han and Hsu, Po-Chun and Lee, Hung-Yi},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{baevski2020vq,
  title     = {{vq-wav2vec}: Self-supervised learning of discrete speech representations},
  author    = {Baevski, Alexei and Schneider, Steffen and Auli, Michael},
  booktitle = {ICLR},
  year      = {2020}
}

@inproceedings{pascual2019learning,
  title     = {Learning problem-agnostic speech representations from multiple self-supervised tasks},
  author    = {Pascual, Santiago and Ravanelli, Mirco and Serra, Joan and Bonafonte, Antonio and Bengio, Yoshua},
  booktitle = {Interspeech},
  year      = {2019}
}

@inproceedings{baevski2020wav2vec,
  title     = {wav2vec 2.0: A framework for self-supervised learning of speech representations},
  author    = {Baevski, Alexei and Zhou, Henry and Mohamed, Abdelrahman and Auli, Michael},
  booktitle = {NeurIPS},
  year      = {2020}
}

@inproceedings{baevski2020effectiveness,
  title     = {Effectiveness of self-supervised pre-training for {ASR}},
  author    = {Baevski, Alexei and Mohamed, Abdelrahman},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{chung2019unsupervised,
  title     = {An unsupervised autoregressive model for speech representation learning},
  author    = {Chung, Yu-An and Hsu, Wei-Ning and Tang, Hao and Glass, James},
  booktitle = {Interspeech},
  year      = {2019}
}

@inproceedings{chung2020improved,
  title     = {Improved speech representations with multi-target autoregressive predictive coding},
  author    = {Chung, Yu-An and Glass, James},
  booktitle = {ACL},
  year      = {2020}
}

@inproceedings{chung2020generative,
  title     = {Generative pre-training for speech with autoregressive predictive coding},
  author    = {Chung, Yu-An and Glass, James},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{schneider2019wav2vec,
  title     = {wav2vec: Unsupervised pre-training for speech recognition},
  author    = {Schneider, Steffen and Baevski, Alexei and Collobert, Ronan and Auli, Michael},
  booktitle = {Interspeech},
  year      = {2019}
}

@inproceedings{song2020speech,
  title     ={{Speech-XLNet}: Unsupervised acoustic model pretraining for self-attention networks},
  author    = {Song, Xingchen and Wang, Guangsen and Wu, Zhiyong and Huang, Yiheng and Su, Dan and Yu, Dong and Meng, Helen},
  booktitle = {Interspeech},
  year      = { 2020}
}

@inproceedings{chung2020vector,
  title     = {Vector-quantized autoregressive predictive coding},
  author    = {Chung, Yu-An and Tang, Hao and Glass, James},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{ling2020deep,
  title     = {Deep contextualized acoustic representations for semi-supervised speech recognition},
  author    = {Ling, Shaoshi and Liu, Yuzong and Salazar, Julian and Kirchhoff, Katrin},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{nguyen2020investigating,
  title     = {Investigating self-supervised pre-training for end-to-end speech translation},
  author    = {Nguyen, Ha and Bougares, Fethi and Tomashenko, Natalia and Est{\`e}ve, Yannick and Besacier, Laurent},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{wu2020self,
  title     = {Self-supervised representations improve end-to-end speech translation},
  author    = {Wu, Anne and Wang, Changhan and Pino, Juan and Gu, Jiatao},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{wu2020defense,
  title     = {Defense for black-box attacks on anti-spoofing models by self-supervised learning},
  author    = {Wu, Haibin and Liu, Andy and Lee, Hung-Yi},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{ravi2020exploring,
  title     = {Exploring the use of an unsupervised autoregressive model as a shared encoder for text-dependent speaker verification},
  author    = {Ravi, Vijay and Fan, Ruchao and Afshan, Amber and Lu, Huanhua and Alwan, Abeer},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{shim2019self,
  title     = {Self-supervised pre-training with acoustic configurations for replay spoofing detection},
  author    = {Shim, Hye-jin and Heo, Hee-Soo and Jung, Jee-weon and Yu, Ha-Jin},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{feng2020unsupervised,
  title     = {Unsupervised subword modeling using autoregressive pretraining and cross-lingual phone-aware modeling},
  author    = {Feng, Siyuan and Scharenborg, Odette},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{kornblith2019similarity,
  title     = {Similarity of neural network representations revisited},
  author    = {Kornblith, Simon and Norouzi, Mohammad and Lee, Honglak and Hinton, Geoffrey},
  booktitle = {ICML},
  year      = {2019}
}

@inproceedings{belinkov2017analyzing,
  title     = {Analyzing hidden representations in end-to-end automatic speech recognition systems},
  author    = {Belinkov, Yonatan and Glass, James},
  booktitle = {NIPS},
  year      = {2017}
}

@inproceedings{wang2017does,
  title     = {What does the speaker embedding encode?},
  author    = {Wang, Shuai and Qian, Yanmin and Yu, Kai},
  booktitle = {Interspeech},
  year      = {2017}
}

@inproceedings{raghu2017svcca,
  title     = {{SVCCA}: Singular vector canonical correlation analysis for deep learning dynamics and interpretability},
  author    = {Raghu, Maithra and Gilmer, Justin and Yosinski, Jason and Sohl-Dickstein, Jascha},
  booktitle = {NIPS},
  year      = {2017}
}

@inproceedings{kahn2020libri,
  title     = {{Libri-Light}: A benchmark for {ASR} with limited or no supervision},
  author    = {Kahn, Jacob and Rivi{\`e}re, Morgane and Zheng, Weiyi and Kharitonov, Eugene and Xu, Qiantong and Mazar{\'e}, Pierre-Emmanuel and Karadayi, Julien and Liptchinsky, Vitaliy and Collobert, Ronan and Fugen, Christian and Likhomanenko, Tatiana and Synnaeve, Gabriel and Joulin, Armand and Abdelrahman, Mohamed and Dupoux, Emmanuel},
  booktitle = {ICASSP},
  year      = {2020},
}

@inproceedings{park2019specaugment,
  title     = {{SpecAugment}: A simple data augmentation method for automatic speech recognition},
  author    = {Park, Daniel and Chan, William and Zhang, Yu and Chiu, Chung-Cheng and Zoph, Barret and Cubuk, Ekin and Le, Quoc},
  booktitle = {Interspeech},
  year      = {2019}
}

@inproceedings{panayotov2015librispeech,
  title     = {{LibriSpeech}: An {ASR} corpus based on public domain audio books},
  author    = {Panayotov, Vassil and Chen, Guoguo and Povey, Daniel and Khudanpur, Sanjeev},
  booktitle = {ICASSP},
  year      = {2015}
}

@inproceedings{paul1992design,
  title     = {The design for the {Wall Street Journal}-based {CSR} corpus},
  author    = {Paul, Douglas and Baker, Janet},
  booktitle = {Speech and Natural Language Workshop},
  year      = {1992}
}

@techreport{garofolo1993darpa,
  title       = {{DARPA} {TIMIT} acoustic-phonetic continuous speech corpus},
  author      = {Garofolo, John and Lamel, Lori and Fisher, William and Fiscus, Jonathan and Pallett, David and Dahlgren, Nancy},
  year        = {1993},
  institution = {NIST},
  number      = {NISTIR 4930}
}

@misc{kawakami2020unsupervised,
  title  = {Unsupervised learning of efficient and robust speech representations},
  author = {Kawakami, Kazuya and Wang, Luyu and Dyer, Chris and Blunsom, Phil and van den Oord, Aaron},
  year   = {2020},
  url    = {https://openreview.net/forum?id=HJe-blSYvH}
}

@inproceedings{kreuk2020self,
  title     = {Self-supervised contrastive learning for unsupervised phoneme segmentation},
  author    = {Kreuk, Felix and Keshet, Joseph and Adi, Yossi},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{bau2019identifying,
  title     = {Identifying and controlling important neurons in neural machine translation},
  author    = {Bau, Anthony and Belinkov, Yonatan and Sajjad, Hassan and Durrani, Nadir and Dalvi, Fahim and Glass, James},
  booktitle = {ICLR},
  year      = {2019}
}

@inproceedings{andrew2013deep,
  title     = {Deep canonical correlation analysis},
  author    = {Andrew, Galen and Arora, Raman and Bilmes, Jeff and Livescu, Karen},
  booktitle = {ICML},
  year      = {2013}
}

@inproceedings{gutmann2010noise,
  title     = {Noise-contrastive estimation: A new estimation principle for unnormalized statistical models},
  author    = {Gutmann, Michael and Hyv{\"a}rinen, Aapo},
  booktitle = {AISTATS},
  year      = {2010}
}

@inproceedings{peters2018deep,
  title     = {Deep contextualized word representations},
  author    = {Peters, Matthew and Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke},
  booktitle = {NAACL-HLT},
  year      = {2018}
}

@inproceedings{devlin2019bert,
  title     = {{BERT}: Pre-training of deep bidirectional {Transformers}for language understanding},
  author    = {Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristin},
  booktitle = {NAACL-HLT},
  year      = {2019}
}

@inproceedings{chen2020simple,
  title     = {A simple framework for contrastive learning of visual representations},
  author    = {Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle = {ICLR},
  year      = {2020}
}

@inproceedings{harwath2020learning,
  title     = {Learning hierarchical discrete linguistic units from visually-grounded speech},
  author    = {Harwath, David and Hsu, Wei-Ning and Glass, James},
  booktitle = {ICLR},
  year      = {2020}
}

@inproceedings{chrupala2017representations,
  title     = {Representations of language in a model of visually grounded speech signal},
  author    = {Chrupa{\l}a, Grzegorz and Gelderloos, Lieke and Alishahi, Afra},
  booktitle = {ACL},
  year      = {2017}
}

@inproceedings{chuang2020speechbert,
  title     = {{SpeechBERT}: Cross-modal pre-trained language model for end-to-end spoken question answering},
  author    = {Chuang, Yung-Sung and Liu, Chi-Liang and Lee, Hung-Yi and Lee, Lin-Shan},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{harwath2016unsupervised,
  title     = {Unsupervised learning of spoken language with visual context},
  author    = {Harwath, David and Torralba, Antonio and Glass, James},
  booktitle = {NIPS},
  year      = {2016}
}

@inproceedings{wu2020similarity,
  title     = {Similarity analysis of contextual word representation models},
  author    = {Wu, John and Belinkov, Yonatan and Sajjad, Hassan and Durrani, Nadir and Dalvi, Fahim and Glass, James},
  booktitle = {ACL},
  year      = {2020}
}

@inproceedings{shukla2020visually,
  title     = {Visually guided self supervised learning of speech representations},
  author    = {Shukla, Abhinav and Vougioukas, Konstantinos and Ma, Pingchuan and Petridis, Stavros and Pantic, Maja},
  booktitle = {ICASSP},
  year      = {2020},
}

==> Self-Supervised Speech Analysis (ICASSP 2021)/strings-fillname.tex <==
@article{liu2020tera,
  title   = {{TERA}: Self-supervised learning of {Transformer} encoder representation for speech},
  author  = {Liu, Andy and Li, Shang-Wen and Lee, Hung-Yi},
  journal = {arXiv preprint arXiv:2007.06028},
  year    = {2020}
}

@article{oord2018representation,
  title   = {Representation learning with contrastive predictive coding},
  author  = {Oord, Aaron van den and Li, Yazhe and Vinyals, Oriol},
  journal = {arXiv preprint arXiv:1807.03748},
  year    = {2018}
}

@article{khurana2020cstnet,
  title   = {{CSTNet}: Contrastive speech translation network for self-supervised speech representation learning},
  author  = {Khurana, Sameer and Laurent, Antoine and Glass, James},
  journal = {arXiv preprint arXiv:2006.02814},
  year    = {2020}
}

@article{jiang2019improving,
  title   = {Improving {Transformer}-based speech recognition using unsupervised pre-training},
  author  = {Jiang, Dongwei and Lei, Xiaoning and Li, Wubo and Luo, Ne and Hu, Yuxuan and Zou, Wei and Li, Xiangang},
  journal = {arXiv preprint arXiv:1910.09932},
  year    = {2019}
}

@article{jiang2020further,
  title   = {A further study of unsupervised pre-training for {Transformer} based speech recognition},
  author  = {Jiang, Dongwei and Li, Wubo and Zhang, Ruixiong and Cao, Miao and Luo, Ne and Han, Yang and Zou, Wei and Li, Xiangang},
  journal = {arXiv preprint arXiv:2005.09862},
  year    = {2020}
}

@article{kriegeskorte2008representational,
  title   = {Representational similarity analysis-connecting the branches of systems neuroscience},
  author  = {Kriegeskorte, Nikolaus and Mur, Marieke and Bandettini, Peter},
  journal = {Frontiers in Systems Neuroscience},
  volume  = {2},
  pages   = {4},
  year    = {2008}
}

@article{chung2020semi,
  title   = {Semi-supervised speech-language joint pre-training for spoken language understanding},
  author  = {Chung, Yu-An and Zhu, Chenguang and Zeng, Michael},
  journal = {arXiv preprint arXiv:2010.02295},
  year    = {2020}
}

==> refs-fullname.tex <==
@inproceedings{blandon2020analysis,
  title     = {Analysis of predictive coding models for phonemic representation learning in small datasets},
  author    = {Bland{\'o}n, Mar{\'\i}a Andrea Cruz and R{\"a}s{\"a}nen, Okko},
  booktitle = {ICML SAS Workshop},
  year      = {2020}
}

@inproceedings{riviere2020unsupervised,
  title     = {Unsupervised pretraining transfers well across languages},
  author    = {Rivi{\`e}re, Morgane and Joulin, Armand and Mazar{\'e}, Pierre-Emmanuel and Dupoux, Emmanuel},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{wang2020unsupervised,
  title     = {Unsupervised pre-training of bidirectional speech encoders via masked reconstruction},
  author    = {Wang, Weiran and Tang, Qingming and Livescu, Karen},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{liu2020mockingjay,
  title     = {Mockingjay: Unsupervised speech representation learning with deep bidirectional {Transformer} encoders},
  author    = {Liu, Andy and Yang, Shu-Wen and Chi, Po-Han and Hsu, Po-Chun and Lee, Hung-Yi},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{baevski2020vq,
  title     = {{vq-wav2vec}: Self-supervised learning of discrete speech representations},
  author    = {Baevski, Alexei and Schneider, Steffen and Auli, Michael},
  booktitle = {ICLR},
  year      = {2020}
}

@inproceedings{pascual2019learning,
  title     = {Learning problem-agnostic speech representations from multiple self-supervised tasks},
  author    = {Pascual, Santiago and Ravanelli, Mirco and Serra, Joan and Bonafonte, Antonio and Bengio, Yoshua},
  booktitle = {Interspeech},
  year      = {2019}
}

@inproceedings{baevski2020wav2vec,
  title     = {wav2vec 2.0: A framework for self-supervised learning of speech representations},
  author    = {Baevski, Alexei and Zhou, Henry and Mohamed, Abdelrahman and Auli, Michael},
  booktitle = {NeurIPS},
  year      = {2020}
}

@inproceedings{baevski2020effectiveness,
  title     = {Effectiveness of self-supervised pre-training for {ASR}},
  author    = {Baevski, Alexei and Mohamed, Abdelrahman},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{chung2019unsupervised,
  title     = {An unsupervised autoregressive model for speech representation learning},
  author    = {Chung, Yu-An and Hsu, Wei-Ning and Tang, Hao and Glass, James},
  booktitle = {Interspeech},
  year      = {2019}
}

@inproceedings{chung2020improved,
  title     = {Improved speech representations with multi-target autoregressive predictive coding},
  author    = {Chung, Yu-An and Glass, James},
  booktitle = {ACL},
  year      = {2020}
}

@inproceedings{chung2020generative,
  title     = {Generative pre-training for speech with autoregressive predictive coding},
  author    = {Chung, Yu-An and Glass, James},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{schneider2019wav2vec,
  title     = {wav2vec: Unsupervised pre-training for speech recognition},
  author    = {Schneider, Steffen and Baevski, Alexei and Collobert, Ronan and Auli, Michael},
  booktitle = {Interspeech},
  year      = {2019}
}

@inproceedings{song2020speech,
  title     ={{Speech-XLNet}: Unsupervised acoustic model pretraining for self-attention networks},
  author    = {Song, Xingchen and Wang, Guangsen and Wu, Zhiyong and Huang, Yiheng and Su, Dan and Yu, Dong and Meng, Helen},
  booktitle = {Interspeech},
  year      = { 2020}
}

@inproceedings{chung2020vector,
  title     = {Vector-quantized autoregressive predictive coding},
  author    = {Chung, Yu-An and Tang, Hao and Glass, James},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{ling2020deep,
  title     = {Deep contextualized acoustic representations for semi-supervised speech recognition},
  author    = {Ling, Shaoshi and Liu, Yuzong and Salazar, Julian and Kirchhoff, Katrin},
  booktitle = {ICASSP},
  year      = {2020}
}

@inproceedings{nguyen2020investigating,
  title     = {Investigating self-supervised pre-training for end-to-end speech translation},
  author    = {Nguyen, Ha and Bougares, Fethi and Tomashenko, Natalia and Est{\`e}ve, Yannick and Besacier, Laurent},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{wu2020self,
  title     = {Self-supervised representations improve end-to-end speech translation},
  author    = {Wu, Anne and Wang, Changhan and Pino, Juan and Gu, Jiatao},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{wu2020defense,
  title     = {Defense for black-box attacks on anti-spoofing models by self-supervised learning},
  author    = {Wu, Haibin and Liu, Andy and Lee, Hung-Yi},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{ravi2020exploring,
  title     = {Exploring the use of an unsupervised autoregressive model as a shared encoder for text-dependent speaker verification},
  author    = {Ravi, Vijay and Fan, Ruchao and Afshan, Amber and Lu, Huanhua and Alwan, Abeer},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{shim2019self,
  title     = {Self-supervised pre-training with acoustic configurations for replay spoofing detection},
  author    = {Shim, Hye-jin and Heo, Hee-Soo and Jung, Jee-weon and Yu, Ha-Jin},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{feng2020unsupervised,
  title     = {Unsupervised subword modeling using autoregressive pretraining and cross-lingual phone-aware modeling},
  author    = {Feng, Siyuan and Scharenborg, Odette},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{kornblith2019similarity,
  title     = {Similarity of neural network representations revisited},
  author    = {Kornblith, Simon and Norouzi, Mohammad and Lee, Honglak and Hinton, Geoffrey},
  booktitle = {ICML},
  year      = {2019}
}

@inproceedings{belinkov2017analyzing,
  title     = {Analyzing hidden representations in end-to-end automatic speech recognition systems},
  author    = {Belinkov, Yonatan and Glass, James},
  booktitle = {NIPS},
  year      = {2017}
}

@inproceedings{wang2017does,
  title     = {What does the speaker embedding encode?},
  author    = {Wang, Shuai and Qian, Yanmin and Yu, Kai},
  booktitle = {Interspeech},
  year      = {2017}
}

@inproceedings{raghu2017svcca,
  title     = {{SVCCA}: Singular vector canonical correlation analysis for deep learning dynamics and interpretability},
  author    = {Raghu, Maithra and Gilmer, Justin and Yosinski, Jason and Sohl-Dickstein, Jascha},
  booktitle = {NIPS},
  year      = {2017}
}

@inproceedings{kahn2020libri,
  title     = {{Libri-Light}: A benchmark for {ASR} with limited or no supervision},
  author    = {Kahn, Jacob and Rivi{\`e}re, Morgane and Zheng, Weiyi and Kharitonov, Eugene and Xu, Qiantong and Mazar{\'e}, Pierre-Emmanuel and Karadayi, Julien and Liptchinsky, Vitaliy and Collobert, Ronan and Fugen, Christian and Likhomanenko, Tatiana and Synnaeve, Gabriel and Joulin, Armand and Abdelrahman, Mohamed and Dupoux, Emmanuel},
  booktitle = {ICASSP},
  year      = {2020},
}

@inproceedings{park2019specaugment,
  title     = {{SpecAugment}: A simple data augmentation method for automatic speech recognition},
  author    = {Park, Daniel and Chan, William and Zhang, Yu and Chiu, Chung-Cheng and Zoph, Barret and Cubuk, Ekin and Le, Quoc},
  booktitle = {Interspeech},
  year      = {2019}
}

@inproceedings{panayotov2015librispeech,
  title     = {{LibriSpeech}: An {ASR} corpus based on public domain audio books},
  author    = {Panayotov, Vassil and Chen, Guoguo and Povey, Daniel and Khudanpur, Sanjeev},
  booktitle = {ICASSP},
  year      = {2015}
}

@inproceedings{paul1992design,
  title     = {The design for the {Wall Street Journal}-based {CSR} corpus},
  author    = {Paul, Douglas and Baker, Janet},
  booktitle = {Speech and Natural Language Workshop},
  year      = {1992}
}

@techreport{garofolo1993darpa,
  title       = {{DARPA} {TIMIT} acoustic-phonetic continuous speech corpus},
  author      = {Garofolo, John and Lamel, Lori and Fisher, William and Fiscus, Jonathan and Pallett, David and Dahlgren, Nancy},
  year        = {1993},
  institution = {NIST},
  number      = {NISTIR 4930}
}

@misc{kawakami2020unsupervised,
  title  = {Unsupervised learning of efficient and robust speech representations},
  author = {Kawakami, Kazuya and Wang, Luyu and Dyer, Chris and Blunsom, Phil and van den Oord, Aaron},
  year   = {2020},
  url    = {https://openreview.net/forum?id=HJe-blSYvH}
}

@inproceedings{kreuk2020self,
  title     = {Self-supervised contrastive learning for unsupervised phoneme segmentation},
  author    = {Kreuk, Felix and Keshet, Joseph and Adi, Yossi},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{bau2019identifying,
  title     = {Identifying and controlling important neurons in neural machine translation},
  author    = {Bau, Anthony and Belinkov, Yonatan and Sajjad, Hassan and Durrani, Nadir and Dalvi, Fahim and Glass, James},
  booktitle = {ICLR},
  year      = {2019}
}

@inproceedings{andrew2013deep,
  title     = {Deep canonical correlation analysis},
  author    = {Andrew, Galen and Arora, Raman and Bilmes, Jeff and Livescu, Karen},
  booktitle = {ICML},
  year      = {2013}
}

@inproceedings{gutmann2010noise,
  title     = {Noise-contrastive estimation: A new estimation principle for unnormalized statistical models},
  author    = {Gutmann, Michael and Hyv{\"a}rinen, Aapo},
  booktitle = {AISTATS},
  year      = {2010}
}

@inproceedings{peters2018deep,
  title     = {Deep contextualized word representations},
  author    = {Peters, Matthew and Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke},
  booktitle = {NAACL-HLT},
  year      = {2018}
}

@inproceedings{devlin2019bert,
  title     = {{BERT}: Pre-training of deep bidirectional {Transformers}for language understanding},
  author    = {Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristin},
  booktitle = {NAACL-HLT},
  year      = {2019}
}

@inproceedings{chen2020simple,
  title     = {A simple framework for contrastive learning of visual representations},
  author    = {Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle = {ICLR},
  year      = {2020}
}

@inproceedings{harwath2020learning,
  title     = {Learning hierarchical discrete linguistic units from visually-grounded speech},
  author    = {Harwath, David and Hsu, Wei-Ning and Glass, James},
  booktitle = {ICLR},
  year      = {2020}
}

@inproceedings{chrupala2017representations,
  title     = {Representations of language in a model of visually grounded speech signal},
  author    = {Chrupa{\l}a, Grzegorz and Gelderloos, Lieke and Alishahi, Afra},
  booktitle = {ACL},
  year      = {2017}
}

@inproceedings{chuang2020speechbert,
  title     = {{SpeechBERT}: Cross-modal pre-trained language model for end-to-end spoken question answering},
  author    = {Chuang, Yung-Sung and Liu, Chi-Liang and Lee, Hung-Yi and Lee, Lin-Shan},
  booktitle = {Interspeech},
  year      = {2020}
}

@inproceedings{harwath2016unsupervised,
  title     = {Unsupervised learning of spoken language with visual context},
  author    = {Harwath, David and Torralba, Antonio and Glass, James},
  booktitle = {NIPS},
  year      = {2016}
}

@inproceedings{wu2020similarity,
  title     = {Similarity analysis of contextual word representation models},
  author    = {Wu, John and Belinkov, Yonatan and Sajjad, Hassan and Durrani, Nadir and Dalvi, Fahim and Glass, James},
  booktitle = {ACL},
  year      = {2020}
}

@inproceedings{shukla2020visually,
  title     = {Visually guided self supervised learning of speech representations},
  author    = {Shukla, Abhinav and Vougioukas, Konstantinos and Ma, Pingchuan and Petridis, Stavros and Pantic, Maja},
  booktitle = {ICASSP},
  year      = {2020},
}

==> strings-fillname.tex <==
@article{liu2020tera,
  title   = {{TERA}: Self-supervised learning of {Transformer} encoder representation for speech},
  author  = {Liu, Andy and Li, Shang-Wen and Lee, Hung-Yi},
  journal = {arXiv preprint arXiv:2007.06028},
  year    = {2020}
}

@article{oord2018representation,
  title   = {Representation learning with contrastive predictive coding},
  author  = {Oord, Aaron van den and Li, Yazhe and Vinyals, Oriol},
  journal = {arXiv preprint arXiv:1807.03748},
  year    = {2018}
}

@article{khurana2020cstnet,
  title   = {{CSTNet}: Contrastive speech translation network for self-supervised speech representation learning},
  author  = {Khurana, Sameer and Laurent, Antoine and Glass, James},
  journal = {arXiv preprint arXiv:2006.02814},
  year    = {2020}
}

@article{jiang2019improving,
  title   = {Improving {Transformer}-based speech recognition using unsupervised pre-training},
  author  = {Jiang, Dongwei and Lei, Xiaoning and Li, Wubo and Luo, Ne and Hu, Yuxuan and Zou, Wei and Li, Xiangang},
  journal = {arXiv preprint arXiv:1910.09932},
  year    = {2019}
}

@article{jiang2020further,
  title   = {A further study of unsupervised pre-training for {Transformer} based speech recognition},
  author  = {Jiang, Dongwei and Li, Wubo and Zhang, Ruixiong and Cao, Miao and Luo, Ne and Han, Yang and Zou, Wei and Li, Xiangang},
  journal = {arXiv preprint arXiv:2005.09862},
  year    = {2020}
}

@article{kriegeskorte2008representational,
  title   = {Representational similarity analysis-connecting the branches of systems neuroscience},
  author  = {Kriegeskorte, Nikolaus and Mur, Marieke and Bandettini, Peter},
  journal = {Frontiers in Systems Neuroscience},
  volume  = {2},
  pages   = {4},
  year    = {2008}
}

@article{chung2020semi,
  title   = {Semi-supervised speech-language joint pre-training for spoken language understanding},
  author  = {Chung, Yu-An and Zhu, Chenguang and Zeng, Michael},
  journal = {arXiv preprint arXiv:2010.02295},
  year    = {2020}
}
